Effect of Timing Error: A Case Study of Navigation Camera

We focus on the problem of timing errors in navigation camera as a case study in a broader problem of the effect of a timing error in cyber-physical systems. These systems rely on the requirement that certain things happen at the same time or certain things happen periodically at some period $T$. However, as these systems get more complex, timing errors can occur between the components thereby violating the assumption about events being simultaneous (or periodic). We consider the problem of a surgical navigation system where optical markers detected in the 2D pictures taken by two cameras are used to localize the markers in 3D space. A predefined array of such markers, known as a reference element, is used to navigate the corresponding CAD model of a surgical instrument on patient's images. The cameras rely on the assumption that the pictures from both cameras are taken exactly at the same time. If a timing error occurs then the instrument may have moved between the pictures. We find that, depending upon the location of the instrument, this can lead to a substantial error in the localization of the instrument. Specifically, we find that if the actual movement is $\delta$ then the observed movement may be as high as $5\delta$ in the operating range of the camera. Furthermore, we also identify potential issues that could affect the error in case there are changes to the camera system or to the operating range.

==> tableraw-data.tex <==


\begin{table}[h]
\tiny
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        &	-50 & -40 & -30 & -20 & -10 & 0 & 10 & 20 & 30 & 40 & 50\\
        \hline
10 & 0.207191 & 0.158908 & 0.112365 & 0.071066 & 0.0502513 & 0.071066 & 0.112365 & 0.158908 & 0.207191 & 0.256232 & 0.305666\\
        \hline

20 & 0.22473 & 0.181183 & 0.142132 & 0.112365 & 0.100503 & 0.112365 & 0.142132 & 0.181183 & 0.22473 & 0.270611 & 0.317817\\        \hline


30 & 0.251256 & 0.213198 & 0.181183 & 0.158908 & 0.150754 & 0.158908 & 0.181183 & 0.213198 & 0.251256 & 0.293013 & 0.337096\\
\hline
40 & 0.284264 & 0.251256 & 0.22473 & 0.207191 & 0.201005 & 0.207191 & 0.22473 & 0.251256 & 0.284264 & 0.321765 & 0.362367\\
        \hline
50 & 0.321765 & 0.293013 & 0.270611 & 0.256232 & 0.251256 & 0.256232 & 0.270611 & 0.293013 & 0.321765 & 0.35533 & 0.392475\\
        \hline
60 & 0.362367 & 0.337096 & 0.317817 & 0.305666 & 0.301508 & 0.305666 & 0.317817 & 0.337096 & 0.362367 & 0.392475 & 0.426396\\
        \hline
70 & 0.405139 & 0.382702 & 0.365835 & 0.35533 & 0.351759 & 0.35533 & 0.365835 & 0.382702 & 0.405139 & 0.432278 & 0.463294\\
        \hline
80 & 0.449461 & 0.429347 & 0.414382 & 0.405139 & 0.40201 & 0.405139 & 0.414382 & 0.429347 & 0.449461 & 0.474069 & 0.502513\\
        \hline
90 & 0.494917 & 0.476725 & 0.463294 & 0.455044 & 0.452261 & 0.455044 & 0.463294 & 0.476725 & 0.494917 & 0.517368 & 0.54355\\
        \hline
100 & 0.541223 & 0.524639 & 0.512464 & 0.505019 & 0.502513 & 0.505019 & 0.512464 & 0.524639 & 0.541223 & 0.561826 & 0.586025\\
 \hline
    \end{tabular}
    \caption{Calculated Error Given dx=0.1, dy=0}
    \label{tab:dx0.1}
\end{table}

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.5]{locationerrordx=0.1dy=0.pdf}
    \caption{Location Error given dx=0.1,dy=0}
    \label{fig:dx0.1}
\end{figure}

\begin{table}[]
\tiny
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        & -50& -40& -30& -20& -10& 0& 10& 20& 30& 40& 50\\ \hline 
10& 1.26218& 0.802609& 0.451731& 0.213198& 0.1& 0.0703589& 0& 0.155777& 0.404226& 0.746198& 1.18112\\ \hline 
  
20& 0.677596& 0.4541& 0.284264& 0.168125& 0.1& 0.0557623& 0& 0.0894678& 0.221393& 0.398901& 0.623109\\ \hline 
  
30& 0.503356& 0.35533& 0.241174& 0.158378& 0.1& 0.0526169& 0& 0.0703589& 0.165563& 0.289138& 0.442786\\ \hline 
  
40& 0.426396& 0.313676& 0.224167& 0.15481& 0.1& 0.0514745& 0& 0.0622665& 0.140718& 0.238626& 0.357871\\ \hline 
  
50& 0.38573& 0.292425& 0.215838& 0.153124& 0.1& 0.0509393& 0& 0.0581351& 0.127552& 0.211077& 0.310547\\ \hline 
  
60& 0.361761& 0.280209& 0.21117& 0.152196& 0.1& 0.0506475& 0& 0.0557623& 0.119786& 0.194446& 0.281436\\ \hline 
  
70& 0.346515& 0.272576& 0.208301& 0.151631& 0.1& 0.0504716& 0& 0.0542821& 0.114847& 0.18368& 0.262291\\ \hline 
  
80& 0.336251& 0.267502& 0.206413& 0.151262& 0.1& 0.0503576& 0& 0.0533001& 0.111525& 0.176336& 0.249066\\ \hline 
  
90& 0.329026& 0.263963& 0.205107& 0.151007& 0.1& 0.0502798& 0& 0.0526169& 0.109189& 0.171119& 0.239572\\ \hline 
  
100& 0.323757& 0.2614& 0.204165& 0.150824& 0.1& 0.0502243& 0& 0.0521233& 0.107488& 0.167287& 0.23254\\ \hline  
          
    \end{tabular}
    \caption{Location Error given dx=0, dy=0.1}
    \label{tab:dy0.1}
\end{table}

